Boosting Diffusion Guidance via Learning Degradation-Aware Models for Blind Super Resolution

Recently, diffusion-based blind super-resolution (SR) methods have shown great ability to generate high-resolution images with abundant high-frequency detail, but the detail is often achieved at the expense of fidelity. Meanwhile, another line of research focusing on rectifying the reverse process of diffusion models (i.e., diffusion guidance), has demonstrated the power to generate high-fidelity results for non-blind SR. However, these methods rely on known degradation kernels, making them difficult to apply to blind SR. To address these issues, we present DADiff in this paper. DADiff incorporates degradation-aware models into the diffusion guidance framework, eliminating the need to know degradation kernels. Additionally, we propose two novel techniques: input perturbation and guidance scalar, to further improve our performance. Extensive experimental results show that our proposed method has superior performance over state-of-the-art methods on blind SR benchmarks.

==> experiments.tex <==
\input{table/DIV2K_quantitative}
\section{Experiments}
\subsection{Experiment Settings}
\label{sec:settings}
% \subsubsection{Data preparation}
% \label{sec:dataset}
\heading{Data preparation.} We evaluate our method on three different dataset, which is DIV2K unknown degradation dataset \cite{Agustsson_2017_CVPR_Workshops}, CelebA-HQ dataset~\cite{liu2015faceattributes} and the ImageNet dataset~\cite{deng2009imagenet}.

% To train the paired degradation and restoration model, we need to generate LR-HR paired data. For DIV2K unknown degradation datastet, the LR-HR pair is provided, we randomly crop corresponding HR patch (resolution: $256 \times 256$) and LR patches (resolution: $64 \times 64$) during the training. For the CelebA and ImageNet dataset, which only contain HR images, we generate corresponding LR images by performing convolutions with random anti-isotropic Gaussian kernels, with the stride equal to the degradation scale. Following Wang \etal \cite{wang2021unsupervised}, we randomly sample a series of parameters of the kernel. Specifically, the filter size is sampled from the odd numbers in the range of $[7, 21]$. The weights are determined by two eigenvalues $\lambda_1$ and $\lambda_2$ of a covariance matrix, both of which are sampled from a uniform distribution $\mathcal{U}(0.2, 4)$. Additionally, we sample a rotation angle $\theta \sim \mathcal{U}(0, \pi)$ to diversify the kernels. Finally, we can use LR-HR pairs to train our degradation and restoration model.

\ren{To train our degradation and restoration models, we generate LR-HR paired data as described in Supplementary.} For testing dataset, We use the official train, test split for DIV2K, following SeeSR \cite{wu2024seesr} we randomly
crop 1K HR patches (resolution: $256 \times 256$) and corresponding LR patches (resolution: $64 \times 64$) from the DIV2K unknown degradation validation set. We name this dataset as \emph{DIV2K-Val}. For the CelebA and ImageNet datasets, we randomly sample 1K images as testing data and generate corresponding LR images using the same pipeline as that for generating training data, naming these testing datasets \emph{CelebA-Val} and \emph{ImageNet-Val}, respectively. We experiment on a 4x degradation scale on \emph{DIV2K-Val}, as only 4x degraded scale LR images are provided officially. For \emph{CelebA-Val} and \emph{ImageNet-Val}, we experiment with both $4 \times$ and $8 \times$ degradation scales.

% \subsubsection{Implementation details}
\heading{Implementation details.} For the \emph{DIV2K-Val} and \emph{ImageNet-Val} testing set, we use the $256 \times 256$ uncondition denoising model pretrained on ImageNet by Dhariwal \etal \cite{dhariwal2021diffusion}. For the CelebA-Val testing set, we use $256 \time 256$ uncondition denoising model pretrained on CelebA release by Meng \etal \cite{meng2021sdedit}. For training the degradation and restoration models, we follow the settings of Li \etal \cite{li2022learning} with the addition of a consistency loss, where the learning rate of the consistency loss is set to $0.1$ of the pixel loss. During inference with the DDNM algorithm, we use DDPM as the diffusion sampling formula and adopt the spaced DDPM sampling \cite{nichol2021improved} with $100$ timesteps. The guidance scalar is set to $0.3$ throughout all the experiments.

% \subsubsection{Compared method}
\heading{Methods in comparison.} We compare our method with several state-of-the-art generative-based blind super-resolution (SR) methods. For the \emph{DIV2K-Val} dataset, we compare our approach with GAN-based methods,  including BSRGAN \cite{zhang2021designing}, Real-ESRGAN \cite{wang2021real}, LDL \cite{liang2022details}, FeMaSR \cite{chen2022real} and DASR \cite{liang2022efficient}. We also compare with diffusion-based methods, including LDM \cite{rombach2022high}, ResShift \cite{yue2024resshift}, PASD \cite{yang2023pixel}, DiffBIR \cite{lin2023diffbir} and SeeSR \cite{wu2024seesr}. For the \emph{CelebA-Val} and \emph{ImageNet-Val} datset, we compare with DiffBIR \cite{lin2023diffbir}, SeeSR \cite{wu2024seesr} and SR3 \cite{saharia2022image}, where SR3 is trained with the same training dataset we use in this work. Since our method is strongly related to \cite{wang2022zero} and MsdiNet \cite{li2022learning}, we also compare it with them. It is worth mentioning that for blind-SR tasks, the ground truth degradation kernel is unknown. Therefore, we use the default SR $\mathbf{A}$ $\mathbf{A}^\dagger$ settings in DDNM experiments, where $\mathbf{A}$ is set to average pooling and $\mathbf{A}^\dagger$ is set to patch upsample. We use the publicly released codes and pretrained models (except SR3) of the competing methods for testing.

We employ several evaluation metrics to showcase our model's capability in terms of fidelity and realism. For fidelity measures, we use PSNR and SSIM \cite{wang2004image}. For perceptual quality measures, we use LPIPS \cite{zhang2018unreasonable} and DISTS \cite{ding2020image}. Additionally, we use FID \cite{heusel2017gans} to evaluate the distance between the distributions of original and restored images. These metrics provide a comprehensive evaluation of our model's performance.

\input{table/other_quantitative}

\subsection{Comparison with State-of-the-Arts}
% \subsubsection{Quantitative comparisons}
\heading{Quantitative comparisons.} We first present the quantitative comparison on \emph{DIV2K-Val} in \cref{tab:div2k}. The following observations can be made: 
1) Compared to DDNM, where $\mathbf{A}$ is set to average pooling and $\mathbf{A}^\dagger$ is set to patch upsample, our method excels in all metrics, showcasing its effectiveness.
2) Our method achieves the best scores on LPIPS, DISTS, and FID metrics, indicating that we effectively utilize the capabilities of pretrained diffusion models to produce outputs with high image quality. Additionally, we achieve the best PSNR and SSIM scores compared to other generative-based blind-SR methods, successfully addressing the challenge that the fidelity weakness often associated with generative-based blind-SR methods. 
3) While MsdiNet has the best scores on fidelity metrics, it performs poorly on perceptual measurements. This is due to its DNN regression-based fidelity-focused learning objectives, which fall short in striking a balance between fidelity and realism. 
Overall, compared with other generative-based blind-SR methods, our method achieves better results not only in fidelity but also in image quality measurements.

We then present the quantitative comparison on \emph{CelebA-Val} and \emph{ImageNet-Val} in \cref{tab:quantitative}. Our method achieves the best scores in image quality measurements. MsdiNet performs best in fidelity but poorly in realism. It's worth noting that although DDNM outperforms our method in fidelity in the ImageNet-Val setting, it still performs poorly on image quality due to the mismatch between $\mathbf{A}$ $\mathbf{A}^\dagger$ and $\mathbf{A}_\text{gt}$. We believe our method strikes a better balance between fidelity and realism compared to DNN regression-based methods (MsdiNet) or other generative-based blind-SR methods.

\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figure/DIV2K_Q.pdf}
    \caption{\heading{Qualitative comparison of $\bf{4 \times}$ upsampling on \emph{DIV2K-Val}.} The magnified areas are indicated with red boxes.}
    \label{fig:div2k_qualitative}
\end{figure*}


% \subsubsection{Qualitative results}

\heading{Qualitative comparisons.} \cref{fig:div2k_qualitative} presents visual comparisons between our method and other diffusion-based blind-SR methods on \emph{DIV2K-Val} dataset. LDM and ResShift produce blurry results since they rely solely on the condition of low-resolution observations without the help of pretrained diffusion priors. DiffBIR and SeeSR can produce outputs with better image quality but often generate incorrect textures due to hallucinations from the diffusion prior. PASD results are blurry due to the challenge of correctly extracting semantic prompts from low-resolution patches. In comparison, our method, with the help of additional degradation and restoration models, can produce outputs that excel in both fidelity and image quality.

\cref{fig:celeba_qualitative} presents visual comparisons between our method and other diffusion-based blind-SR methods on the \emph{CelebA-Val} dataset. SR3 generates excessive high-frequency information. DiffBIR and SeeSR exhibit shortcomings in fidelity. DDNM, without ground truth $\mathbf{A}$ $\mathbf{A}^\dagger$, and MsdiNet struggle to generate high-quality images. In contrast, our method, with the assistance of degradation and restoration models, achieves high fidelity and image quality.



\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figure/CelebA_Q.pdf}
    \caption{\heading{Qualitative comparison of $\bf{4 \times}$ upsampling on \emph{CelebA-Val}.} Zoomed LR use bicubic upsample.}
    \label{fig:celeba_qualitative}
\end{figure*}


\input{table/ablation}

\subsection{Ablation Studies}
% \subsubsection{Effectiveness of input perturbation and guidance scalar}
\heading{Effectiveness of input perturbation and guidance scalar.} To demonstrate the impact of input perturbation and the guidance scalar, we conducted detailed ablation studies on our proposed method using the \emph{DIV2K-Val}, \emph{CelebA-Val}, and \emph{ImageNet-Val} datasets, as summarized in \cref{tab:ablation}. We compared the results of simply combining DDNM \cite{wang2022zero} with the extra degradation and restoration models against incorporating input perturbation, the guidance scalar, or both. The addition of the guidance scalar led to significant improvements in both fidelity and image quality. For fidelity measurement, it increased PSNR by 7.2 dB in the \emph{DIV2K-Val} dataset, 2.2 dB in the \emph{CelebA-Val} dataset, and 3.5 dB in the \emph{ImageNet-Val} dataset. For image quality measurement, it increased LPIPS by 0.27 in the \emph{DIV2K-Val} dataset, 0.03 in the \emph{CelebA-Val} dataset, and 0.1 in the \emph{ImageNet-Val} dataset. Similarly, the inclusion of input perturbation also improved both fidelity and realism. Importantly, combining both techniques further enhanced the overall results, underscoring the effectiveness of these strategies in boosting the performance of our method.


% \subsubsection{How to model degradation operator and its pseudo-inverse}
\heading{How to model degradation operator and its pseudo-inverse.} We conducted experiments using various approaches to model the degradation operator and its corresponding pseudo-inverse. Results are presented in \cref{tab:differentA}. We trained a DNN regression-based degradation and restoration model to approximate $\mathbf{A}$ $\mathbf{A}^\dagger$ in DDNM \cite{wang2022zero} algorithm, providing a more generalized approach to modeling the degradation and its corresponding pseudo-inverse. In our ablation experiments, we refer to this method as \emph{implicit}, as the degradation representation is implicitly learned as a feature. Another naive approach to modeling the degradation operator and its pseudo-inverse is by defining $\mathbf{A}$ as a convolution with an explicit Gaussian kernel. This method assumes $\mathbf{A}$ is linear and known, allowing $\mathbf{A}^\dagger$ to be calculated using techniques like Singular Value Decomposition (SVD), similar to what DDNM proposes. However, relying on the assumption that $\mathbf{A}$ is a convolution operator limits its expressiveness compared to methods that learn the degradation implicitly or through more complex models.

To construct an experiment based on this approach, we trained an explicit kernel estimator using the same training data described in \cref{sec:settings}. Given a low-resolution input observation, the explicit kernel estimator predicts a corresponding explicit linear degradation kernel. We define convolution with the predicted kernel as $\mathbf{A}$ and calculate its corresponding pseudo-inverse operator $\mathbf{A}^\dagger$ using SVD. In our ablation study, we refer to this method as \emph{explicit} as it explicitly defines the degradation process using a Gaussian kernel. To further experiment with the modularization of $\mathbf{A}$ $\mathbf{A}^\dagger$ in DDNM \cite{wang2022zero} algorithm, we also explore combining the explicit version of $\mathbf{A}$ with the implicit version of $\mathbf{A}^\dagger$. In our ablation study, we refer to this approach as \emph{combine}.

In \cref{tab:differentA}, we observe that for the \emph{DIV2K-Val} and \emph{ImageNet-Val} datasets, the implicit version of $\mathbf{A}$ $\mathbf{A}^\dagger$ outperforms the \emph{combine} and \emph{explicit} approaches. This superiority is attributed to the greater expressiveness of the implicit degradation representation compared to convolution with a Gaussian kernel. Convolution with a Gaussian kernel assumes a global degradation operator, which limits its ability to capture variations in degradation that can occur locally across an image in real-world scenarios. It's worth mention that even with a global degradation operator, the actual degradation level can vary significantly due to differences in the content of the original image.


On the \emph{CelebA-Val} dataset, we observe that the explicit setting of $\mathbf{A}$ $\mathbf{A}^\dagger$ performs better than the \emph{combine} and \emph{implicit} approaches. This can be attributed to \emph{CelebA-Val} being a less complex dataset, where the expressiveness of convolution with a Gaussian kernel is sufficient to model the degradation observed in the low-resolution inputs. Additionally, the explicit setting benefits from having $\mathbf{A}^\dagger$ as the perfect pseudo-inverse of $\mathbf{A}$, calculated via SVD. In general, the explicit setting works well when the degradation can be approximated by a linear kernel, allowing for the perfect pseudo-inverse relationship between$\mathbf{A}$ $\mathbf{A}^\dagger$. On the other hand, the implicit setting of $\mathbf{A}$ $\mathbf{A}^\dagger$ offers better expressiveness in modeling degradation, which makes our method more robust and reliable across diverse datasets and real-world scenarios.

\input{table/differentA}

% \subsubsection{Ablation study on the value of guidance scalar}

\heading{Ablation study on the value of guidance scalar.} Note that the guidance scalar $\alpha$ in \cref{eq:alpha_guidance}
 is a crucial parameter. If $\alpha$ is set too high, it accelerates the restoration process, leading to the hallucination problem in the pretrained diffusion model. Conversely, setting it too low reduces the influence of the guidance, leading to low fidelity output. Note that setting it to zero equates to unconditional diffusion sampling. We conduct an ablation study on the value of the guidance scalar, as shown in \cref{tab:scalar_ablation}. %Additionally, Patashnik \etal \cite{patashnik2023localizing} have highlighted that the denoising process of pretrained diffusion models inherently follows a coarse-to-fine synthesis, affecting the layout, subject shape, and visual details generation towards the end. Accelerating the restoration process may introduce undesired inputs to the diffusion model at various timesteps. However, 
 By introducing the guidance scalar \(\sim [0, 1]\), we effectively slow down the restoration process, thereby mitigating the performance decrease caused by restoration acceleration. %\cref{tab:scalar_ablation} demonstrates the beneficial impact of the alpha scalar in improving the overall performance of our method.





==> table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}

\begin{table*}[]
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c|ccccccccccccc}
\multicolumn{1}{l|}{Matrics} & MsdiNet                        & BSRGAN  & \begin{tabular}[c]{@{}c@{}}Real-\\ ESRGAN\end{tabular} & LDL     & DASR    & FeMaSR  & DDNM     & LDM                            & ResShift                      & PASD    & DiffBIR  & SeeSR   & ours                           \\ \hline
PSNR ↑                       & {\color[HTML]{FF0000} 27.3933} & 22.0694 & 21.7337                                                & 23.1245 & 22.9961 & 20.2219 & 23.0214  & 21.7728                        & 21.6208                       & 22.7452 & 20.7647  & 21.8206 & {\color[HTML]{0000FF} 24.4681} \\
SSIM ↑                       & {\color[HTML]{FF0000} 0.7276}  & 0.5188  & 0.5179                                                 & 0.5355  & 0.5369  & 0.4601  & 0.5459   & 0.5108                         & 0.5101                        & 0.5348  & 0.4422   & 0.5009  & {\color[HTML]{0000FF} 0.6208}  \\
LPIPS ↓                      & 0.3486                         & 0.3392  & 0.3486                                                 & 0.3498  & 0.3682  & 0.3242  & 0.4814   & 0.3238                         & {\color[HTML]{0000FF} 0.3097} & 0.412   & 0.4106   & 0.3399  & {\color[HTML]{FF0000} 0.3069}  \\
DISTS ↓                      & 0.2558                         & 0.2634  & 0.2681                                                 & 0.2746  & 0.2824  & 0.2573  & 0.3182   & {\color[HTML]{0000FF} 0.2474}  & 0.2543                        & 0.2855  & 0.2866   & 0.2599  & {\color[HTML]{FF0000} 0.2393}  \\
FID ↓                        & 91.772                         & 92.604  & 91.3774                                                & 94.2726 & 102.948 & 94.2519 & 106.1603 & {\color[HTML]{0000FF} 83.9125} & 88.3887                       & 90.0368 & 101.1623 & 86.939  & {\color[HTML]{FF0000} 82.2803}
\end{tabular}
\end{adjustbox}
\caption{DIV2k blind quantitative result}
\label{tab:div2k}
\end{table*}




\begin{table*}[]
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{cc|ccccc|ccccc}
\multicolumn{2}{c|}{scale}                                     & \multicolumn{5}{c|}{x4}                                                                                                                                         & \multicolumn{5}{c}{x8}                                                                                                                                          \\ \hline
\multicolumn{1}{c|}{Dataset}                         & Method  & PSNR ↑                         & SSIM ↑                        & LPIPS ↓                       & DISTS ↓                       & FID ↓                          & PSNR ↑                         & SSIM ↑                        & LPIPS ↓                       & DISTS ↓                       & FID ↓                          \\ \hline
\multicolumn{1}{c|}{}                                & DDNM    & 25.6975                        & {\color[HTML]{0000FF} 0.8069} & 0.2074                        & 0.1634                        & 38.3359                        & 20.1491                        & 0.65                          & 0.2469                        & 0.2061                        & 52.6844                        \\
\multicolumn{1}{c|}{}                                & SR3     & 26.0082                        & 0.7392                        & {\color[HTML]{0000FF} 0.1289} & {\color[HTML]{0000FF} 0.1209} & {\color[HTML]{0000FF} 19.4323} & 23.79                          & {\color[HTML]{0000FF} 0.6995} & {\color[HTML]{0000FF} 0.1742} & {\color[HTML]{0000FF} 0.1505} & {\color[HTML]{0000FF} 25.6039} \\
\multicolumn{1}{c|}{}                                & DiffBIR & 22.9068                        & 0.7098                        & 0.1769                        & 0.1793                        & 66.8081                        & 19.0676                        & 0.5621                        & 0.264                         & 0.2102                        & 67.7493                        \\
\multicolumn{1}{c|}{}                                & SeeSR   & 22.3977                        & 0.7187                        & 0.1808                        & 0.1747                        & 66.7649                        & 19.2302                        & 0.5827                        & 0.2542                        & 0.1974                        & 67.6858                        \\
\multicolumn{1}{c|}{}                                & MsdiNet & {\color[HTML]{FF0000} 28.8877} & {\color[HTML]{FF0000} 0.8317} & 0.2405                        & 0.2048                        & 59.757                         & {\color[HTML]{FF0000} 25.2789} & {\color[HTML]{FF0000} 0.7527} & 0.3426                        & 0.2555                        & 76.6328                        \\
\multicolumn{1}{c|}{\multirow{-6}{*}{celeba\_val}}   & ours    & {\color[HTML]{0000FF} 27.1513} & 0.7784                        & {\color[HTML]{FF0000} 0.0913} & {\color[HTML]{FF0000} 0.1066} & {\color[HTML]{FF0000} 18.6689} & {\color[HTML]{0000FF} 22.8065} & 0.6893                        & {\color[HTML]{FF0000} 0.1502} & {\color[HTML]{FF0000} 0.1399} & {\color[HTML]{FF0000} 23.9716} \\ \hline
\multicolumn{1}{c|}{}                                & DDNM    & {\color[HTML]{0000FF} 23.1482} & {\color[HTML]{0000FF} 0.6792} & 0.4273                        & 0.2364                        & {\color[HTML]{0000FF} 61.4687} & {\color[HTML]{0000FF} 18.9643} & {\color[HTML]{0000FF} 0.5246} & 0.5655                        & 0.3084                        & 102.1028                       \\
\multicolumn{1}{c|}{}                                & SR3     & 17.8748                        & 0.5645                        & 0.3218                        & 0.2291                        & 95.9887                        & 17.0792                        & 0.4807                        & 0.4288                        & 0.2686                        & 126.1097                       \\
\multicolumn{1}{c|}{}                                & DiffBIR & 20.311                         & 0.5583                        & {\color[HTML]{0000FF} 0.2986} & {\color[HTML]{0000FF} 0.2186} & 65.1268                        & 17.2329                        & 0.4168                        & {\color[HTML]{0000FF} 0.4252} & {\color[HTML]{0000FF} 0.2662} & {\color[HTML]{0000FF} 89.7597} \\
\multicolumn{1}{c|}{}                                & SeeSR   & 19.9072                        & 0.5692                        & 0.3022                        & 0.2232                        & 66.0386                        & 17.3075                        & 0.4329                        & 0.4317                        & 0.2744                        & 95.8495                        \\
\multicolumn{1}{c|}{}                                & MsdiNet & {\color[HTML]{FF0000} 24.6502} & {\color[HTML]{FF0000} 0.6979} & 0.4006                        & 0.2669                        & 97.8515                        & {\color[HTML]{FF0000} 21.593}  & {\color[HTML]{FF0000} 0.5857} & 0.5487                        & 0.3404                        & 151.5809                       \\
\multicolumn{1}{c|}{\multirow{-6}{*}{imagenet\_val}} & ours    & 22.3551                        & 0.6006                        & {\color[HTML]{FF0000} 0.2673} & {\color[HTML]{FF0000} 0.1896} & {\color[HTML]{FF0000} 47.548}  & 18.6632                        & 0.4507                        & {\color[HTML]{FF0000} 0.4117} & {\color[HTML]{FF0000} 0.2558} & {\color[HTML]{FF0000} 79.2494}
\end{tabular}
\end{adjustbox}
\caption{celeba, imagenet quantitative result}
\label{tab:quantitative}
\end{table*}




\begin{table*}[]
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{cc|ccc|ccc|ccc}
\hline
\multicolumn{2}{c|}{dataset}                                                                                               & \multicolumn{3}{c|}{div2k}                                                                     & \multicolumn{3}{c|}{celeba}                                                                    & \multicolumn{3}{c}{imagenet}                                                                   \\ \hline
\begin{tabular}[c]{@{}c@{}}input \\ perturbation\end{tabular} & \begin{tabular}[c]{@{}c@{}}guidance \\ scalar\end{tabular} & PSNR ↑                         & SSIM ↑                        & LPIPS ↓                       & PSNR ↑                         & SSIM ↑                        & LPIPS ↓                       & PSNR ↑                         & SSIM ↑                        & LPIPS ↓                       \\ \hline
v                                                             & v                                                          & {\color[HTML]{FF0000} 24.4681} & {\color[HTML]{FF0000} 0.6208} & {\color[HTML]{FF0000} 0.3069} & {\color[HTML]{FF0000} 27.1513} & {\color[HTML]{FF0000} 0.7784} & {\color[HTML]{FF0000} 0.0913} & {\color[HTML]{FF0000} 22.3551} & {\color[HTML]{FF0000} 0.6006} & {\color[HTML]{FF0000} 0.2673} \\
-                                                             & v                                                          & {\color[HTML]{0000FF} 20.7559} & {\color[HTML]{0000FF} 0.5525} & {\color[HTML]{0000FF} 0.3544} & {\color[HTML]{0000FF} 26.727}  & {\color[HTML]{0000FF} 0.7724} & {\color[HTML]{0000FF} 0.0939} & {\color[HTML]{0000FF} 21.5244} & {\color[HTML]{0000FF} 0.5784} & {\color[HTML]{0000FF} 0.2732} \\
v                                                             & -                                                          & 17.5641                        & 0.3585                        & 0.5147                        & 26.1626                        & 0.7575                        & 0.1002                        & 20.4946                        & 0.5235                        & 0.2981                        \\
-                                                             & -                                                          & 13.5803                        & 0.2281                        & 0.6269                        & 24.5115                        & 0.7145                        & 0.1247                        & 18.0744                        & 0.4212                        & 0.3821                        \\ \hline
\end{tabular}
\end{adjustbox}
\caption{ablation result}
\label{tab:ablation}
\end{table*}




\begin{table}[]
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c|c|ccc}
\hline
dataset                                                                     & method   & PSNR                           & SSIM                          & LPIPS                         \\ \hline
                                                                            & implicit & {\color[HTML]{FF0000} 24.4681} & {\color[HTML]{FF0000} 0.6208} & {\color[HTML]{FF0000} 0.3069} \\
                                                                            & explicit & 20.955                         & 0.3999                        & 0.5985                        \\
\multirow{-3}{*}{DIV2K-Val}                                                 & combine  & 22.4154                        & 0.531                         & 0.4787                        \\ \hline
                                                                            & implicit & 27.1513                        & 0.7784                        & 0.0913                        \\
                                                                            & explicit & {\color[HTML]{FF0000} 28.4252} & {\color[HTML]{FF0000} 0.8173} & {\color[HTML]{FF0000} 0.0874} \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}CelebA-Val\\ x4\end{tabular}}   & combine  & 27.5289                        & 0.7953                        & 0.0935                        \\ \hline
                                                                            & implicit & {\color[HTML]{FF0000} 22.3551} & {\color[HTML]{FF0000} 0.6006} & {\color[HTML]{FF0000} 0.2673} \\
                                                                            & explicit & 20.5606                        & 0.4596                        & 0.5699                        \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}ImageNet-Val\\ x4\end{tabular}} & combine  & 21.5035                        & 0.5999                        & 0.308                         \\ \hline
\end{tabular}
\end{adjustbox}
\caption{comparing explicit, implicit and combine}
\label{tab:differentA}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c|clll}
\hline
dataset                                                                    & method    & \multicolumn{1}{c}{PSNR}    & \multicolumn{1}{c}{SSIM}   & \multicolumn{1}{c}{LPIPS}  \\ \hline
\multirow{5}{*}{DIV2K-Val}                                                 & alpha=0.1 &                             &                            &                            \\
                                                                           & alpha=0.2 &                             &                            &                            \\
                                                                           & alpha=0.3 & \multicolumn{1}{c}{20.7559} & \multicolumn{1}{c}{0.5525} & \multicolumn{1}{c}{0.3544} \\
                                                                           & alpha=0.5 &                             &                            &                            \\
                                                                           & alpha=1.0 & \multicolumn{1}{c}{13.5803} & \multicolumn{1}{c}{0.2281} & \multicolumn{1}{c}{0.6269} \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}CelebA-Val\\ x4\end{tabular}}   & alpha=0.1 &                             &                            &                            \\
                                                                           & alpha=0.2 &                             &                            &                            \\
                                                                           & alpha=0.3 & \multicolumn{1}{c}{26.727}  & \multicolumn{1}{c}{0.7724} & \multicolumn{1}{c}{0.0939} \\
                                                                           & alpha=0.5 &                             &                            &                            \\
                                                                           & alpha=1.0 & \multicolumn{1}{c}{24.5115} & \multicolumn{1}{c}{0.7145} & \multicolumn{1}{c}{0.1247} \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}ImageNet-Val\\ x4\end{tabular}} & alpha=0.1 &                             &                            &                            \\
                                                                           & alpha=0.2 &                             &                            &                            \\
                                                                           & alpha=0.3 & \multicolumn{1}{c}{21.5244} & \multicolumn{1}{c}{0.5784} & \multicolumn{1}{c}{0.2732} \\
                                                                           & alpha=0.5 &                             &                            &                            \\
                                                                           & alpha=1.0 & \multicolumn{1}{c}{18.0744} & \multicolumn{1}{c}{0.4212} & \multicolumn{1}{c}{0.3821} \\ \hline
\end{tabular}
\end{adjustbox}
\caption{ablation study on value of guidance scalar}
\label{tab:scalar_ablation}
\end{table}
